Securing the Management Plane in Intent-based Cellular Networks

IBN is an emerging network management paradigm that allows automated closed-loop control and management of network devices and services. Closed-loop control requires security primitives to avoid intrusive human impact on network policies, posing a serious security challenge. This paper addresses this critical problem by securing the management plane in IBN systems. We propose a novel security framework based on WireGuard that augments the existing standards to secure intent communication between intent stakeholders. The framework guarantees isolation through WireGuard tunnels and provides inherent authentication and access control mechanisms to avoid intrusion in IBN systems. This work contributes to developing secure, efficient, and flexible communication channels within the IBN ecosystem, ensuring the integrity and confidentiality of network intents and operational data. Experimental results show the suitability and superiority of WireGuard compared to OpenVPN.

==> Resources/Algorithm/noise_hs.tex <==
\begin{algorithm}
\caption{Key Exchange between CSC and IBNSC using Noise protocol}
\label{algo:noise_hs}
\begin{algorithmic}[1]
\State \textbf{CSC} and \textbf{IBNSC} have static key pairs $(s_I, S_I)$ and $(s_R, S_R)$ \{$s_x$: private key, $S_x$: public key\}, where $x = {I, R}$
\State CSC knows $S_R$ in advance
\State CSC generates ephemeral key pair $(e_I, E_I)$
\State CSC computes 
\Statex $DH_1 = DH(e_I, S_R)$, $DH_2 = DH(s_I, S_R)$

\State CSC encrypts $S_I$ using $DH_1$, $DH_2$
\State CSC $\xrightarrow{E_I, \text{encrypted}(S_I)}$ R
\State IBNSC generates ephemeral key pair $(e_R, E_R)$
\State IBNSC computes
\Statex $DH_1, DH_2, DH_3 = DH(s_R, E_I)$, 
\Statex $DH_4 = DH(e_R, S_I)$, 
\Statex $DH_5 = DH(e_R, E_I)$

\State IBNSC $\xrightarrow{E_R}$ CSC
\State CSC computes $DH_3, DH_4, DH_5$
\State Both CSC and IBNSC derive symmetric keys from $DH_1, DH_2, DH_3, DH_4, DH_5$
\end{algorithmic}
\end{algorithm}

==> Resources/Tables/openstack-resources.tex <==
\begin{table}[htbp]
\centering
\caption{OpenStack implementation of the stakeholders.}
\label{tab:openstack-resources}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{Stakeholder} & \textbf{OS} & \textbf{vCPUs} & \textbf{RAM (GB)} & \textbf{Storage (GB)} \\
\hline
IBNSC & Ubuntu 22.04 & 4 & 16 & 40 \\
CSC & Ubuntu 22.04 & 4 & 16 & 40 \\
CSP & Ubuntu 22.04 & 4 & 16 & 40 \\
NOP & Ubuntu 22.04 & 4 & 16 & 40 \\
VISP & Ubuntu 22.04 & 4 & 16 & 40 \\
\hline
\end{tabular}%
}
\end{table}

==> Resources/Tables/vpn-comp.tex <==
\begin{table}[h!]
\centering
\begin{tabular}{|>{\raggedright\arraybackslash}p{3cm}|>{\raggedright\arraybackslash}p{4cm}|>{\raggedright\arraybackslash}p{4cm}|>{\raggedright\arraybackslash}p{4cm}|}
\hline
\textbf{Feature} & \textbf{WireGuard} & \textbf{OpenVPN} & \textbf{IPsec} \\
\hline
\textbf{Design} & Simple, fast, secure & Highly configurable, versatile & Suite of protocols for securing IP communications \\
\hline
\textbf{Transport} & UDP & UDP and TCP & Network layer (Layer 3) \\
\hline
\textbf{Encryption Algorithms} & ChaCha20, Poly1305, Curve25519 & AES, Blowfish, Camellia & AES, 3DES, others \\
\hline
\textbf{Key Generation} & Curve25519 & SSL/TLS (RSA, ECDSA) & IKE (RSA, ECDSA) \\
\hline
\textbf{Key Exchange} & Noise Protocol Framework & SSL/TLS & IKE (Internet Key Exchange) \\
\hline
\textbf{Forward Secrecy} & Yes, through periodic key rotation & Yes, through TLS session resumption and renegotiation & Yes, through IKEv2 and Perfect Forward Secrecy (PFS) \\
\hline
\textbf{Key Rotation Protocols} & Periodic key rotation (e.g., every few minutes) & TLS session resumption and renegotiation & IKEv2 with periodic rekeying \\
\hline
\textbf{Performance} & Optimized for high performance and low latency & Generally good performance, but can be slower & Generally good performance, but can be slower \\
\hline
\textbf{Pros} & Simple, fast, modern cryptography, small codebase & Highly configurable, supports both UDP and TCP, well-established & Operates at the network layer, robust security features, well-established \\
\hline
\textbf{Cons} & Fewer features, less mature & More complex, larger codebase, potentially slower & More complex, larger codebase, potentially slower \\
\hline
\end{tabular}
\caption{Comparison of WireGuard, OpenVPN, and IPsec}
\label{tab:vpn_comparison}
\end{table}

==> Resources/Tables/vpn-comp1.tex <==
\begin{table*}[ht]
\centering
\caption{Comparison of WireGuard, OpenVPN, and IPsec}
\begin{tabular}{|p{3.5cm}|p{3.5cm}|p{3.5cm}|p{3.5cm}|}
\hline
\textbf{Criteria}                & \textbf{WireGuard}                                                  & \textbf{OpenVPN}                                                   & \textbf{IPsec}                                                   \\
\hline
\textbf{Protocol}                & Custom protocol based on Noise protocol                & SSL/TLS-based protocol (OpenSSL)                   & Set of protocols (AH, ESP, IKE) based on IP layer \\
\hline
\textbf{Encryption Algorithms}   & ChaCha20, Poly1305, Curve25519                         & AES, RSA, Blowfish, and many others                & AES, 3DES, Blowfish, RSA, and others              \\
\hline
\textbf{Speed/Performance}       & Very fast, minimal overhead                            & Moderate performance, higher overhead due to SSL/TLS & Varies; moderate to high with hardware acceleration \\
\hline
\textbf{Security}                & Strong modern cryptography, streamlined by default     & Very secure, highly configurable                    & Very secure, but complex configuration required    \\
\hline
\textbf{Ease of Setup}           & Easy to set up, minimal configuration                  & More complex, requires certificates/config files   & Complex setup, especially for large deployments    \\
\hline
\textbf{Port Usage}              & Single UDP port (default: 51820)                      & Customizable; uses both TCP and UDP                & Standard ports (UDP 500 for IKE, 4500 for NAT)    \\
\hline
\textbf{Connection Establishment}& Quick, stateless design                                & Slower, TLS handshakes introduce latency           & Slower, due to complex negotiation process         \\
\hline
\textbf{Cross-Platform Support}  & Supported on Linux, Windows, macOS, iOS, Android      & Supported on almost all OS and devices             & Supported widely, especially in enterprise setups  \\
\hline
\textbf{Mobility \& Roaming}     & Excellent; IP changes handled well                    & Moderate support                                   & Can be problematic with network changes            \\
\hline
\textbf{NAT Traversal}           & Good NAT traversal                                     & Good with UDP, complex with TCP                    & Requires special handling for NAT traversal        \\
\hline
\textbf{Battery Efficiency}      & Efficient, low overhead for mobile devices             & Power-intensive due to encryption workload         & Power-hungry; not ideal for mobile devices         \\
\hline
\textbf{Auditability}            & Small codebase, around 4,000 lines, easier to audit    & Large codebase, harder to audit                    & Mature but complex; auditing is more difficult     \\
\hline
\textbf{Use Case Scenarios}      & Ideal for personal use, mobile, and SMBs              & Flexible for various scenarios and enterprises     & Enterprise, site-to-site VPNs                     \\
\hline
\textbf{License}                 & GPLv2                                                 & GPLv2                                              & Open standards, implementations vary               \\
\hline
\textbf{Maturity}                & Newer, rapidly growing adoption                        & Mature, widely used                                & Very mature, a traditional standard                \\
\hline
\end{tabular}
\end{table*}
